Boundary Nevanlinna-Pick interpolation via reduction and augmentation

We give an elementary proof of Sarason's solvability criterion for the Nevanlinna-Pick problem with boundary interpolation nodes and boundary target values. We also give a concrete parametrization of all solutions of such a problem. The proofs are based on a reduction method due to Julia and Nevanlinna. Reduction of functions corresponds to Schur complementation of the corresponding Pick matrices.

==> bdrNP.bbl.tex <==

\begin{thebibliography}{9}% Replace 9 by 99 if 10 or more references
\bibitem{ball} 
J. A. Ball,  Interpolation problems of Pick-Nevanlinna and Loewner types for meromorphic matrix functions, {\em Integral equ. oper. theory}, {\bf 6} (1983) 804-840.

\bibitem{bgr}
J. A. Ball, I. Gohberg and L. Rodman, {\em Interpolation of Rational Matrix Functions}, Operator Theory: Advances and Applications Vol. 45, Birkh\"auser Verlag, Basel, 1990.

\bibitem{bh}
J. A. Ball and J. W. Helton,  Interpolation problems of Pick-Nevanlinna and Loewner types for meromorphic matrix functions: parametrization of the set of all solutions. {\em Integral equ. oper. theory}, {\bf 9} (1986) 155--203.

\bibitem{BD}
V. Bolotnikov and H. Dym,  On boundary interpolation for matrix valued Schur functions, {\em AMS Memoirs} {\bf 181} (2006) Number 856, 1-107.

\bibitem{Bolot} V. Bolotnikov and A. Kheifets,
The higher-order Carath\'eodory-Julia theorem and related boundary interpolation problems,
 in  {\em Recent advances in matrix and operator theory}, Operator Theory: Advances and Applications Vol. 179,  63--102,  Birkh\"auser, Basel, 2008.

\bibitem{Donoghue}
 W. F. Donoghue Jr, {\em Monotone matrix functions and analytic continuation}, Springer Verlag,  Berlin 1974.

\bibitem{Geo}
D. R. Georgijevi\'c, Solvability condition for a boundary value interpolation problem of Loewner type, {\em J. Analyse Math\'ematique}, {\bf 74} (1998) 213-234.

\bibitem{Ju20} 
G. Julia,  Extension nouvelle d'un lemme de Schwarz, {\em Acta Math.}, {\bf 42} (1920) 349-355.

\bibitem{ko89}
I. V. Kovalishina, A multiple boundary value interpolation problem for contracting matrix functions in the unit disk (Russian)  {\em Teor. Funktsii Funktsional. Anal. Prilozhen. } {\bf 51}  (1989) 38--55; translation in {\em J. Soviet Math.} {\bf 52} (1990) 3467--3481.

\bibitem{Mar}
D. E. Marshall,   An elementary proof of the Pick-Nevanlinna interpolation theorem,
{\em Michigan Math. J.}, {\bf  21} (1975), 219-223.

\bibitem{Nev1}
R. Nevanlinna, Kriterien f\"ur die Randwerte beschr\"{a}nkter Funktionen, {\em Math. Zeitschrift} {\bf 13} (1922) 1-9.

\bibitem{S}
D. Sarason, Nevanlinna-Pick interpolation with boundary data, {\em Integr. equ. oper. theory}, {\bf 30} (1998) 231-250.

\bibitem{S2}
D. Sarason, {\em Sub-Hardy Hilbert spaces in the unit disk}, University of Arkansas Lecture Notes in the Mathematical Sciences, John Wiley and Sons, New York 1994.

\bibitem{wig}
E. Wigner,  On a class of analytic functions from the quantum theory of collisions, {\em Ann. Maths}, {\bf 53} (1951) 36-59.
\end{thebibliography}


